Regression with Observational Multilayered Network Data

A novel method to estimate social effect coefficients in the popular so-called linear-in-means regression model in the Social Sciences is presented here that utilizes non-experimental multidimensional network data. The procedure can accommodate social interactions that correlate with the error in the model by making use of a different set of network links among the same observations that are exogenous in the traditional sense. In particular, the full observability of a two-layered multiplex network data structure is assumed here to propose a new Generalized 3-Stage Least Squares (G3SLS) estimator that is consistent, asymptotically normally distributed, and also easy to implement using widely-used existing statistical software because of its closed-form definition. The underlying assumptions are general enough to accommodate common problems with observational data such as measurement error, simultaneity, and unobserved heterogeneity. Monte Carlo exercises confirm the good small sample performance of the proposed G3SLS estimator in these scenarios. An empirical application finds positive and significant peer effects in citations among research articles published in top general-interest journals in economics.

==> gph/tochange_bp.tex <==

%Change:

%\begin{groupplot}[group style={group size=3 by 6, vertical sep=0.2cm}]
ytick style={color=black}

% Add in groupplot 16, 17 and 18:

xtick style={color=black},
xtick = {1.5,4.5,7.5},
xticklabels = {$n = 50$,$n = 100$,$n = 200$}

% Delete in those same groups:

xtick \empty 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Add to qq plot only for gamma

ylabel= Sample Quantiles,
y label style={at={(axis description cs:1.7,0.5)},rotate=0,anchor=south}

==> model.tex <==
\subsection{Econometric Specification}

To quantify the existence of positive human capital externalities or peer effects among scholars publishing in these T4 journals, a linear-in-means social interaction model analogous to the model in (\ref{E1}) is used:

\begin{eqnarray}
  y_{ij}&=&\alpha+\beta\sum_{r=1}^{n}\mathbf{W}_{ir}y_{rj}+\delta\sum_{r=1}^{n}\mathbf{W}_{ir}\mathbf{x}_{rj}+\gamma \mathbf{x}_{ij}+\varepsilon_{ij}\text{,}\label{est_eq} \\
  \varepsilon_{ij}&=&\zeta_{j}+\lambda_{W}+u_{ij}\text{,} \nonumber
\end{eqnarray}

where $y_{ij}$ is the the number published articles of scholar $i$ in journal $j$, $\mathbf{W}$ is a $2,057\times 2,057$ adjacency matrix of all scholars under consideration with $\mathbf{W}_{ij}=1/n_{i}$ if scholars $i$ and $j$ are coauthors and zero otherwise. The exogenous covariates $\mathbf{x}_{ij}$ include \texttt{InCharge}$_{cli}$ which take the value of one if scholar $i$ is in-charge of a journal $j$, and \texttt{Editor}$_i$ which equals one if scholar $i$ has ever been an editor across the observation periods in any T4 journal. The latter's inclusion serves two purposes, it controls for the time-invariant quality of the network, and to account for the fact that the data set does not contain publishing outcomes for the editors. These exogenous variables are also used as the basis to construct a set of instrumental variables allowing the identification of the social effects as suggested in section \ref{indet}.

There are two important elements in the composite error $\varepsilon_{ij}$. First, journals may posses unobserved characteristics that facilitate the publication process for some scholars, for instance, journals may have different tastes for some topics which would affect the ability of some researchers to publish in those journals. The specification in ($\ref{est_eq}$) allows that possibility by including $\zeta_{j}$ in the composite error. To control that, the estimation of this linear-in-means model includes journals fixed effects. Probably more problematic is the unobserved feature $\lambda_{W}$ related with both the number of papers that a scholar can potentially publish and her ability to create coauthorship connections. To tackle this potential endogeneity issue, the estimation of the social parameters use the predetermined variation coming from the \textit{Same Ph.D.} network $\mathbf{W}_{0}$. Initially, the identifying assumption is that $\mathbf{W}_{0}$ is not correlated with $\lambda_{W}$ but it can be relaxed by implementing the transformed model presented in \ref{indet}.

\begin{figure}[H]
\centering
\caption{Visualization of Academic Links between Editors and Published Papers' Authors}\label{backup}
\includegraphics[width=1\textwidth]{project_1/gph/Fig_net.eps}
    \begin{minipage}{1\textwidth}
    \footnotesize
    Dark blue nodes represent the editors in charge in the years 2000, 2003, and 2006 of the American Economic Review (AER), Econometrica (ECA), the Journal of Political Economy (JPE), and the Quarterly Journal of Economics (QJE). All remaining nodes represent each article published that year, where the light blue nodes represent articles where at least one of their authors' held a professional academic link (gray straight lines) with the editors in charge. White nodes represent articles where none of the authors held an observable professional link with the editors. Nodes are ordered clockwise (starting at the second quarter) by their degree (number of connections).
    \end{minipage}
\end{figure}

\begin{figure}[H]
\centering
\caption{Networks Visualization}\label{backup_info}
\vspace{-15mm}
\includegraphics[width=1\textwidth]{project_1/gph/Fig_W_pool.eps}
    \begin{minipage}{1\textwidth}
\vspace{-15mm}
    \footnotesize
    `Nodes' represent all scholars (authors and editors) for all four journals (AER, ECA, JPE, and QJE) in all time periods (2000--2006). `Edges' refer to the total number of connections between them. `Density' is defined as the ratio of the number of edges to the number of possible edges in these networks. `Degree' stands for the average degree, i.e., the average number of edges connected to each node, while `Clust. Coef.' stands for the average clustering coefficient of a node, i.e., the ratio of existing links connecting a node's neighbors to each other to the maximum possible number of such links.
    \end{minipage}
\end{figure}\clearpage 

==> results.tex <==
The first set of results are for the social parameters in the model represented by equation (\ref{est_eq}) without applying any transformation to the model. Considering that the proposed estimator is designed for cross=sectional data, all the coefficients will be calculated for each year in the sample by using a cumulative procedure. For the year 2000, the sample is formed by the number publications of the 2,057 scholars, and the \texttt{InCharge} variable equals one for the editors in charge of one of the T4 journals in that year. For the year 2001, the sample is composed by the same 2,057 scholars but the number of publications is the sum of the publications in 2000 and 2001. Similarly, for that year, the \texttt{InCharge} variable equals one if the editor was in charge of the journals in 2000 or 2001. The process continues in the same way until it arrives to 2006. 

\begin{figure}[H]
\centering
\caption{Peer Effects in Number of Publications}\label{Fig3}
\vspace{-5mm}
\includegraphics[width=0.85\textwidth]{fig_pe.eps}
    \begin{minipage}{0.9\textwidth}
\vspace{0mm}
    \footnotesize
    The dependent variable is the number of published articles. The peer effects coefficients are estimated by using the procedure proposed in section \ref{est}. The standard errors are calculated using the cluster version of equation (\ref{E23}), where the clustering is performed at the journal level. The sample for each year is 2,057 scholars and the number of publications is accumulated year by year.  
    \end{minipage}
\end{figure}

\begin{figure}[H]
\centering
\caption{Exogenous Social Effects in Number of Publications}\label{Fig4}
\vspace{-5mm}
\includegraphics[width=0.85\textwidth]{fig_ed.eps}
    \begin{minipage}{0.9\textwidth}
\vspace{0mm}
    \footnotesize
    The dependent variable is the number of published articles. The peer effects coefficients are estimated by using the procedure proposed in section \ref{est}. The standard errors are calculated using the cluster version of equation (\ref{E23}), where the clustering is performed at the journal level. The sample for each year is 2,057 scholars and the number of publications is accumulated year by year. 
    \end{minipage}
\end{figure}


Figure \ref{Fig3} shows the estimated peer effects coefficients by the procedure proposed in section \ref{est}. The black lines represent the 95\% confidence interval calculated with the standard errors in equation (\ref{E23}) cluster at the journal level. Figure \ref{Fig4}, presents the same information for the editorial contextual parameters.

The first relevant set of results is related with the peer effect among scholars. This new estimation procedure finds a positive relationship between the coauthorship professional network structure and research publication outcomes. Under the identifying assumptions, this positive result reflects human capital spillovers that act through a variety of mechanisms. These mechanisms are found in cases where researchers provide feedback on each other's work, serve as referees, and work together as coauthors. These instances of collaboration are often paramount to the extension of existing research agendas and can bring to light novel ideas. The peer effects coefficient is persistently positive, but it is significant only for the years 2000, 2005 and 2006. 

Note that the peer effects coefficients rank from 0.101 to 0.172. In words, increasing the average number of publications of individual $i$'s set of coauthors, increases her number of publications from 0.101 to 0.172 papers. This may seem empirically non significant. However, considering that the average number of publications is 0.392 for the aggregate value in 2006, the peer effects coefficients represent an increase ranging between 26\% and 44\% of the average of total publications.


A second important result is the positive and significant coefficient of the proportion of scholar $i$'s coauthors who are editors in charge on their total number of publications. To remark is the positive time tendency of the \texttt{Incharge} coefficient. Considering that this variable aggregates more editors in charge each year, scholars will potentially have more coauthors who are in charge of T4 journals. Then, if the effect of that variable is positive, the coefficient should be increasing for every year that passes. Also relevant is that, the effect of the proportion of of scholar $i$'s coauthors who are editors (but not in charge) does not have a significant effect. This may be an indication that what matters is not to have connections who have been editors, but those who have been editors in charge. 

Quantitatively, the effect of the \texttt{Incharge} variable ranges from 0.1 to 0.41, while the one for \texttt{Editor}  is between 0.05 and 0.69. As a percentage of the average of total publications, these coefficients represent an increase of 25\% to 97\%, and 14\% to 175\% for the \texttt{Incharge} and \texttt{Editor} coefficients respectively.

Some studies have interpreted findings similar to the one just presented as favoritism in the publication process. However, the fact that after controlling for peer effects and potential endogenous network formation, the contextual effect of \texttt{Incharge} is still positive, it does not necessarily implies favoritism. Different mechanisms like signaling, searching or complementarties existing between editors and authors can be acting when analyzing why and who publishes in these top journals.

The fact that the editor coefficient is not significant can be an argument against the signaling explanation. Editors are among the top scholars in the profession and a connection to any of them may signal unobserved attributes of the author. If signaling is the mechanism driving the results, the coefficients of the proportion of editors in scholars reference groups would be expected to be positive and significant. Another possible mechanism like learning effects would also predict a positive an significant editors effect. Differentiating between searching and favoritism explanations is more complicated and left for future research.

==> tables/design1_heterogeneity_app1.tex <==
\begin{table}[!htbp]
\centering
\small
\caption{Estimator Performance under Unobserved Degree Heterogeneity}
\label{tab:design1_heterogeneity_app1}
\begin{tabular}{ccc c cccc c cccc c cccc}
\toprule
 &  &  &  &\multicolumn{4}{c}{Peer effects} &  &\multicolumn{4}{c}{Contextual effects} &  &\multicolumn{4}{c}{Direct effects} \\
\cmidrule(lr){5-8} \cmidrule(lr){10-13} \cmidrule(lr){15-18}
$m$ & Estimator & $n$ &  & Bias & SD & RMSE & IQR &  & Bias & SD & RMSE & IQR &  & Bias & SD & RMSE & IQR \\
\midrule
\multirow{9}{*}{\textbf{10}} & \multirow{3}{*}{\textbf{OLS}} & \textbf{50} &  & 0.359 & 0.046 & 0.361 & 0.072 &  & -1.119 & 0.875 & 1.420 & 1.357 &  & -0.449 & 0.616 & 0.762 & 0.983 \\
 &  & \textbf{100} &  & 0.352 & 0.031 & 0.353 & 0.049 &  & -1.104 & 0.576 & 1.245 & 0.897 &  & -0.441 & 0.417 & 0.607 & 0.643 \\
 &  & \textbf{200} &  & 0.348 & 0.022 & 0.349 & 0.033 &  & -1.110 & 0.404 & 1.181 & 0.633 &  & -0.472 & 0.287 & 0.552 & 0.442 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G2SLS}} & \textbf{50} &  & 0.691 & 0.317 & 0.760 & 0.306 &  & -1.612 & 2.233 & 2.754 & 2.917 &  & -0.588 & 1.087 & 1.235 & 1.502 \\
 &  & \textbf{100} &  & 0.742 & 0.268 & 0.789 & 0.278 &  & -2.143 & 1.786 & 2.789 & 2.500 &  & -0.816 & 0.811 & 1.150 & 1.158 \\
 &  & \textbf{200} &  & 0.810 & 0.272 & 0.854 & 0.289 &  & -2.532 & 1.551 & 2.969 & 2.203 &  & -1.034 & 0.714 & 1.256 & 0.957 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G3SLS}} & \textbf{50} &  & 0.074 & 0.986 & 0.989 & 1.283 &  & 0.250 & 6.687 & 6.689 & 8.261 &  & 0.500 & 1.594 & 1.670 & 2.372 \\
 &  & \textbf{100} &  & 0.027 & 0.773 & 0.773 & 1.032 &  & 0.214 & 4.136 & 4.140 & 5.281 &  & 0.562 & 1.079 & 1.217 & 1.629 \\
 &  & \textbf{200} &  & -0.005 & 0.549 & 0.549 & 0.791 &  & 0.245 & 2.486 & 2.497 & 3.500 &  & 0.562 & 0.718 & 0.912 & 1.124 \\
\midrule
\multirow{9}{*}{\textbf{12}} & \multirow{3}{*}{\textbf{OLS}} & \textbf{50} &  & 0.361 & 0.047 & 0.364 & 0.074 &  & -1.132 & 1.043 & 1.539 & 1.628 &  & -0.454 & 0.736 & 0.865 & 1.163 \\
 &  & \textbf{100} &  & 0.354 & 0.031 & 0.355 & 0.050 &  & -1.110 & 0.687 & 1.305 & 1.078 &  & -0.441 & 0.501 & 0.667 & 0.776 \\
 &  & \textbf{200} &  & 0.350 & 0.022 & 0.351 & 0.034 &  & -1.118 & 0.481 & 1.217 & 0.749 &  & -0.476 & 0.344 & 0.588 & 0.533 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G2SLS}} & \textbf{50} &  & 0.732 & 0.304 & 0.793 & 0.305 &  & -1.770 & 2.619 & 3.160 & 3.341 &  & -0.627 & 1.266 & 1.413 & 1.758 \\
 &  & \textbf{100} &  & 0.795 & 0.236 & 0.829 & 0.266 &  & -2.199 & 1.952 & 2.940 & 2.632 &  & -0.840 & 0.914 & 1.241 & 1.371 \\
 &  & \textbf{200} &  & 0.827 & 0.204 & 0.852 & 0.240 &  & -2.543 & 1.541 & 2.974 & 2.249 &  & -1.044 & 0.732 & 1.275 & 0.997 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G3SLS}} & \textbf{50} &  & 0.114 & 1.004 & 1.011 & 1.295 &  & -0.051 & 7.860 & 7.857 & 9.720 &  & 0.473 & 1.902 & 1.959 & 2.851 \\
 &  & \textbf{100} &  & 0.115 & 0.824 & 0.831 & 1.088 &  & -0.069 & 4.997 & 4.995 & 6.546 &  & 0.523 & 1.267 & 1.371 & 1.941 \\
 &  & \textbf{200} &  & 0.015 & 0.608 & 0.608 & 0.832 &  & 0.148 & 2.927 & 2.930 & 4.032 &  & 0.550 & 0.857 & 1.018 & 1.328 \\
\bottomrule
\end{tabular}
\vspace{0.25em}
{\footnotesize
\setstretch{1}
\textit{Notes:} This table reports Monte Carlo results under unobserved degree heterogeneity. The parameter $m$ controls the intensity of heterogeneity in node degrees and is common across individuals. Reported statistics include bias, SD, RMSE, and IQR for the peer ($\beta$), contextual ($\delta$), and direct ($\gamma$) effects. All statistics are computed after symmetric trimming of 10\% in each tail. True parameter values are $\beta = 0.7$, $\delta = 1.0$, and $\gamma = 1.0$.
}
\normalsize
\end{table}

==> tables/design1_heterogeneity_app2.tex <==
\begin{table}[!htbp]
\centering
\small
\caption{Estimator Performance under Unobserved Degree Heterogeneity}
\label{tab:design1_heterogeneity_app2}
\begin{tabular}{ccc c cccc c cccc c cccc}
\toprule
 &  &  &  &\multicolumn{4}{c}{Peer effects} &  &\multicolumn{4}{c}{Contextual effects} &  &\multicolumn{4}{c}{Direct effects} \\
\cmidrule(lr){5-8} \cmidrule(lr){10-13} \cmidrule(lr){15-18}
$m$ & Estimator & $n$ &  & Bias & SD & RMSE & IQR &  & Bias & SD & RMSE & IQR &  & Bias & SD & RMSE & IQR \\
\midrule
\multirow{9}{*}{\textbf{10}} & \multirow{3}{*}{\textbf{OLS}} & \textbf{50} &  & 0.359 & 0.046 & 0.361 & 0.072 &  & -1.119 & 0.875 & 1.420 & 1.357 &  & -0.449 & 0.616 & 0.762 & 0.983 \\
 &  & \textbf{100} &  & 0.352 & 0.031 & 0.353 & 0.049 &  & -1.104 & 0.576 & 1.245 & 0.897 &  & -0.441 & 0.417 & 0.607 & 0.643 \\
 &  & \textbf{200} &  & 0.348 & 0.022 & 0.349 & 0.033 &  & -1.110 & 0.404 & 1.181 & 0.633 &  & -0.472 & 0.287 & 0.552 & 0.442 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G2SLS}} & \textbf{50} &  & 0.691 & 0.317 & 0.760 & 0.306 &  & -1.612 & 2.233 & 2.754 & 2.917 &  & -0.588 & 1.087 & 1.235 & 1.502 \\
 &  & \textbf{100} &  & 0.742 & 0.268 & 0.789 & 0.278 &  & -2.143 & 1.786 & 2.789 & 2.500 &  & -0.816 & 0.811 & 1.150 & 1.158 \\
 &  & \textbf{200} &  & 0.810 & 0.272 & 0.854 & 0.289 &  & -2.532 & 1.551 & 2.969 & 2.203 &  & -1.034 & 0.714 & 1.256 & 0.957 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G3SLS}} & \textbf{50} &  & 0.074 & 0.986 & 0.989 & 1.283 &  & 0.250 & 6.687 & 6.689 & 8.261 &  & 0.500 & 1.594 & 1.670 & 2.372 \\
 &  & \textbf{100} &  & 0.027 & 0.773 & 0.773 & 1.032 &  & 0.214 & 4.136 & 4.140 & 5.281 &  & 0.562 & 1.079 & 1.217 & 1.629 \\
 &  & \textbf{200} &  & -0.005 & 0.549 & 0.549 & 0.791 &  & 0.245 & 2.486 & 2.497 & 3.500 &  & 0.562 & 0.718 & 0.912 & 1.124 \\
\midrule
\multirow{9}{*}{\textbf{12}} & \multirow{3}{*}{\textbf{OLS}} & \textbf{50} &  & 0.361 & 0.047 & 0.364 & 0.074 &  & -1.132 & 1.043 & 1.539 & 1.628 &  & -0.454 & 0.736 & 0.865 & 1.163 \\
 &  & \textbf{100} &  & 0.354 & 0.031 & 0.355 & 0.050 &  & -1.110 & 0.687 & 1.305 & 1.078 &  & -0.441 & 0.501 & 0.667 & 0.776 \\
 &  & \textbf{200} &  & 0.350 & 0.022 & 0.351 & 0.034 &  & -1.118 & 0.481 & 1.217 & 0.749 &  & -0.476 & 0.344 & 0.588 & 0.533 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G2SLS}} & \textbf{50} &  & 0.732 & 0.304 & 0.793 & 0.305 &  & -1.770 & 2.619 & 3.160 & 3.341 &  & -0.627 & 1.266 & 1.413 & 1.758 \\
 &  & \textbf{100} &  & 0.795 & 0.236 & 0.829 & 0.266 &  & -2.199 & 1.952 & 2.940 & 2.632 &  & -0.840 & 0.914 & 1.241 & 1.371 \\
 &  & \textbf{200} &  & 0.827 & 0.204 & 0.852 & 0.240 &  & -2.543 & 1.541 & 2.974 & 2.249 &  & -1.044 & 0.732 & 1.275 & 0.997 \\
\noalign{\vskip 0.5em}
 & \multirow{3}{*}{\textbf{G3SLS}} & \textbf{50} &  & 0.114 & 1.004 & 1.011 & 1.295 &  & -0.051 & 7.860 & 7.857 & 9.720 &  & 0.473 & 1.902 & 1.959 & 2.851 \\
 &  & \textbf{100} &  & 0.115 & 0.824 & 0.831 & 1.088 &  & -0.069 & 4.997 & 4.995 & 6.546 &  & 0.523 & 1.267 & 1.371 & 1.941 \\
 &  & \textbf{200} &  & 0.015 & 0.608 & 0.608 & 0.832 &  & 0.148 & 2.927 & 2.930 & 4.032 &  & 0.550 & 0.857 & 1.018 & 1.328 \\
\bottomrule
\end{tabular}
\vspace{0.25em}
{\footnotesize
\setstretch{1}
\textit{Notes:} This table reports Monte Carlo results under unobserved degree heterogeneity. The parameter $m$ controls the intensity of heterogeneity in node degrees and is common across individuals. Reported statistics include bias, SD, RMSE, and IQR for the peer ($\beta$), contextual ($\delta$), and direct ($\gamma$) effects. All statistics are computed after symmetric trimming of 10\% in each tail. True parameter values are $\beta = 0.7$, $\delta = 1.0$, and $\gamma = 1.0$.
}
\normalsize
\end{table}

==> tbl/W_diff.tex <==
\begin{table}[!htbp]\centering
{
\renewcommand{\arraystretch}{1.25}
\caption{OLS: $\mathbf{W}_n\,\texttt{Different\hspace{0.8mm}Gender}$ on $\mathbf{W}_{n,0}$ regressors}
\label{tab:W_diff}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Variables} & \multicolumn{2}{c}{\textbf{2002}} & \multicolumn{2}{c}{\textbf{2003}} & \multicolumn{2}{c}{\textbf{2004}} & \multicolumn{2}{c}{\textbf{2005}} & \multicolumn{2}{c}{\textbf{2006}} \\
\cmidrule(lr){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
 & Coef. & SE & Coef. & SE & Coef. & SE & Coef. & SE & Coef. & SE \\
\midrule
$\mathbf{W}_{n,0}\ \texttt{log(citation8)}$ & 0.013*** & 0.003 & 0.018*** & 0.004 & 0.021*** & 0.003 & 0.024*** & 0.003 & 0.026*** & 0.003 \\
$\mathbf{W}_{n,0}\ \texttt{Editor}$ & 0.103 & 0.081 & 0.04 & 0.088 & 0.144 & 0.099 & 0.174* & 0.096 & 0.159* & 0.088 \\
$\mathbf{W}_{n,0}\ \texttt{Different\hspace{0.8mm}Gender}$ & 0.142** & 0.058 & 0.172*** & 0.062 & 0.111** & 0.054 & 0.044 & 0.046 & 0.085* & 0.049 \\
\midrule
$n$ & 729 &  & 961 &  & 1187 &  & 1412 &  & 1628 &  \\
$R^2$ & 0.1193 &  & 0.1592 &  & 0.1656 &  & 0.1921 &  & 0.2188 &  \\
$F$ & 18.85 &  & 37.56 &  & 47.12 &  & 45.98 &  & 84.54 &  \\
\bottomrule
\end{tabular}
}
\vspace{0.05cm}
\begin{flushleft}\footnotesize Note: Standard errors (SE)are clustered at the coauthor network component level. $^{*}\,p<0.10$, $^{**}\,p<0.05$, $^{***}\,p<0.01$.\end{flushleft}
\end{table}

==> tbl/W_editor.tex <==
\begin{table}[!htbp]\centering
{
\renewcommand{\arraystretch}{1.25}
\caption{OLS: $\mathbf{W}_n\,\texttt{Editor}$ on $\mathbf{W}_{n,0}$ regressors}
\label{tab:W_editor}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Variables} & \multicolumn{2}{c}{\textbf{2002}} & \multicolumn{2}{c}{\textbf{2003}} & \multicolumn{2}{c}{\textbf{2004}} & \multicolumn{2}{c}{\textbf{2005}} & \multicolumn{2}{c}{\textbf{2006}} \\
\cmidrule(lr){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
 & Coef. & SE & Coef. & SE & Coef. & SE & Coef. & SE & Coef. & SE \\
\midrule
$\mathbf{W}_{n,0}\ \texttt{log(citation8)}$ & 0.009** & 0.004 & 0.013*** & 0.004 & 0.013*** & 0.004 & 0.016*** & 0.004 & 0.014*** & 0.003 \\
$\mathbf{W}_{n,0}\ \texttt{Editor}$ & 0.137 & 0.098 & 0.186* & 0.108 & 0.232** & 0.103 & 0.168** & 0.079 & 0.192*** & 0.071 \\
$\mathbf{W}_{n,0}\ \texttt{Different\hspace{0.8mm}Gender}$ & 0.033 & 0.046 & -0.051 & 0.041 & -0.029 & 0.038 & -0.043 & 0.029 & -0.033 & 0.03 \\
\midrule
$n$ & 729 &  & 961 &  & 1187 &  & 1412 &  & 1628 &  \\
$R^2$ & 0.0806 &  & 0.0963 &  & 0.1079 &  & 0.1252 &  & 0.1348 &  \\
$F$ & 9.82 &  & 13.00 &  & 12.58 &  & 10.09 &  & 10.39 &  \\
\bottomrule
\end{tabular}
}
\vspace{0.05cm}
\begin{flushleft}\footnotesize Note: Standard errors (SE)are clustered at the coauthor network component level. $^{*}\,p<0.10$, $^{**}\,p<0.05$, $^{***}\,p<0.01$.\end{flushleft}
\end{table}

==> tbl/Wy_logcit.tex <==
\begin{table}[!htbp]\centering
{
\renewcommand{\arraystretch}{1.25}
\caption{OLS: $\mathbf{W}_n\,\texttt{log(citation8)}$ on $\mathbf{W}_{n,0}$ regressors}
\label{tab:Wy_logcit}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Variables} & \multicolumn{2}{c}{\textbf{2002}} & \multicolumn{2}{c}{\textbf{2003}} & \multicolumn{2}{c}{\textbf{2004}} & \multicolumn{2}{c}{\textbf{2005}} & \multicolumn{2}{c}{\textbf{2006}} \\
\cmidrule(lr){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
 & Coef. & SE & Coef. & SE & Coef. & SE & Coef. & SE & Coef. & SE \\
\midrule
$\mathbf{W}_{n,0}\ \texttt{log(citation8)}$ & 0.496*** & 0.038 & 0.582*** & 0.036 & 0.624*** & 0.036 & 0.678*** & 0.037 & 0.717*** & 0.042 \\
$\mathbf{W}_{n,0}\ \texttt{Editor}$ & 0.425 & 0.937 & 1.391 & 1.134 & 2.162* & 1.115 & 1.94* & 1.01 & 2.277** & 0.961 \\
$\mathbf{W}_{n,0}\ \texttt{Different\hspace{0.8mm}Gender}$ & 0.137 & 0.574 & -0.024 & 0.476 & -0.151 & 0.491 & -0.532 & 0.438 & -0.723 & 0.455 \\
\midrule
$n$ & 729 &  & 961 &  & 1187 &  & 1412 &  & 1628 &  \\
$R^2$ & 0.4615 &  & 0.5545 &  & 0.6021 &  & 0.6392 &  & 0.6726 &  \\
$F$ & 87.78 &  & 128.99 &  & 145.23 &  & 127.24 &  & 103.55 &  \\
\bottomrule
\end{tabular}
}
\vspace{0.05cm}
\begin{flushleft}\footnotesize Note: Standard errors (SE)are clustered at the coauthor network component level. $^{*}\,p<0.10$, $^{**}\,p<0.05$, $^{***}\,p<0.01$.\end{flushleft}
\end{table}

==> tbl/stats.tex <==
\begin{tabular}{lrrrrrrr}
\hline
             \textbf{Variable} &     2000 &     2001 &     2002 &     2003 &     2004 &     2005 &     2006 \\
\hline
    \textbf{Number of Authors} &    376 &    410 &    486 &    411 &    395 &    410 &    411 \\
                  AER &    136 &    166 &    189 &    168 &    140 &    169 &    172 \\
                  ECA &     93 &    111 &    153 &    107 &    107 &    111 &    108 \\
                  JPE &     87 &     79 &     93 &     80 &     98 &     76 &     71 \\
                  QJE &     74 &     80 &     73 &     80 &     80 &     82 &     84 \\ \hline
  \textbf{Number of Articles} &    221 &    238 &    270 &    232 &    226 &    225 &    216 \\
                  AER &     79 &     88 &     92 &     90 &     79 &     89 &     88 \\
                  ECA &     51 &     64 &     90 &     59 &     61 &     55 &     51 \\
                  JPE &     49 &     44 &     48 &     43 &     46 &     41 &     37 \\
                  QJE &     42 &     42 &     40 &     40 &     40 &     40 &     40 \\ \hline
  \textbf{Number of Citations} &  10,856 &  12,088 &  14,161 &  14,079 &  14,564 &  14,861 &  13,103 \\
                  AER &   4,140 &   4,833 &   4,476 &   4,586 &   5,354 &   5,606 &   5,289 \\
                  ECA &   2,530 &   2,773 &   3,346 &   3,379 &   2,811 &   2,724 &   2,914 \\
                  JPE &   1,692 &   1,446 &   2,240 &   1,954 &   2,787 &   3,420 &   1,852 \\
                  QJE &   2,494 &   3,036 &   4,099 &   4,160 &   3,612 &   3,111 &   3,048 \\ \hline
    \textbf{Number of Editors} &     16 &     20 &     23 &     16 &     18 &     24 &     14 \\
                  AER &      3 &      2 &      7 &      6 &      4 &      8 &      9 \\
                  ECA &      4 &      9 &      5 &      3 &      8 &      2 &      3 \\
                  JPE &      4 &      2 &      7 &      4 &      3 &      7 &      1 \\
                  QJE &      5 &      7 &      4 &      3 &      3 &      7 &      1 \\ \hline
     \textbf{Number of Pages} &   5,486 &   5,984 &   6,870 &   6,327 &   6,356 &   6,529 &   5,979 \\
                  AER &   1,409 &   1,537 &   1,557 &   1,636 &   1,589 &   1,702 &   1,807 \\
                  ECA &   1,297 &   1,566 &   2,341 &   1,735 &   1,772 &   1,877 &   1,559 \\
                  JPE &   1,337 &   1,379 &   1,424 &   1,396 &   1,429 &   1,397 &   1,131 \\
                  QJE &   1,443 &   1,502 &   1,548 &   1,560 &   1,566 &   1,553 &   1,482 \\ \hline
 \textbf{Number of References} &   7,042 &   7,425 &   8,426 &   7,633 &   7,645 &   8,115 &   7,141 \\
                  AER &   2,420 &   2,783 &   2,729 &   2,896 &   2,576 &   3,032 &   2,888 \\
                  ECA &   1,388 &   1,695 &   2,598 &   1,772 &   2,013 &   1,886 &   1,467 \\
                  JPE &   1,285 &   1,311 &   1,452 &   1,391 &   1,503 &   1,445 &   1,166 \\
                  QJE &   1,949 &   1,636 &   1,647 &   1,574 &   1,553 &   1,752 &   1,620 \\ \hline
     \textbf{Different Gender} &     24 &     34 &     37 &     34 &     29 &     27 &     41 \\
                  AER &      7 &     15 &     18 &     16 &      9 &     15 &     21 \\
                  ECA &      7 &      6 &      8 &      5 &      5 &      2 &      9 \\
                  JPE &      4 &      6 &      5 &      5 &      7 &      0 &      3 \\
                  QJE &      6 &      7 &      6 &      8 &      8 &     10 &      8 \\
\hline
\end{tabular}

